Indexability is Not Enough for Whittle: Improved, Near-Optimal Algorithms for Restless Bandits

We study the problem of planning restless multi-armed bandits (RMABs) with multiple actions. This is a popular model for multi-agent systems with applications like multi-channel communication, monitoring and machine maintenance tasks, and healthcare. Whittle index policies, which are based on Lagrangian relaxations, are widely used in these settings due to their simplicity and near-optimality under certain conditions. In this work, we first show that Whittle index policies can fail in simple and practically relevant RMAB settings, even when the RMABs are indexable. We discuss why the optimality guarantees fail and why asymptotic optimality may not translate well to practically relevant planning horizons. We then propose an alternate planning algorithm based on the mean-field method, which can provably and efficiently obtain near-optimal policies with a large number of arms, without the stringent structural assumptions required by the Whittle index policies. This borrows ideas from existing research with some improvements: our approach is hyper-parameter free, and we provide an improved non-asymptotic analysis which has: (a) no requirement for exogenous hyper-parameters and tighter polynomial dependence on known problem parameters; (b) high probability bounds which show that the reward of the policy is reliable; and (c) matching sub-optimality lower bounds for this algorithm with respect to the number of arms, thus demonstrating the tightness of our bounds. Our extensive experimental analysis shows that the mean-field approach matches or outperforms other baselines.

==> backup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Approximation proof written by separating rounding and randomness error.
%% Only done for the rounding error. This is supposed to be used for the
%% Azuma-Hoeffding technique to get better error bounds, as mentioned by
%% Dheeraj.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The real-life state $\rmu_t$ may be different from the mean-field state $\mmu_t$ due to two sources of randomness/approximation: (i) the rounding error when computing $\ralpha_t$ as a function of $\rmu_t$ and $\beta_t$; (ii) the randomness in $\rmu_{t+1}$ given $\rmu_t$ and $\ralpha_t$ due to the stochasticity of the transitions. Notice that the rounding error may be biased and can accumulate over time. Let us denote this bias between the real-life state and mean-field state as $\eta = (\eta_{t,s})$, where $\eta_{t,s} = \Exp[\rmu_{t,s} - \mmu_{t,s} \mid \beta, \mu_1]$. On the other hand, let $\xi = (\xi_{t,s})$ be the unbiased randomness in $\rmu_{t,s}$, defined as: $\xi_{t,s} = \rmu_{t,s} - \mmu_{t,s} - \eta{t,s}$. So, we have decomposed the real-life state into the mean-field state plus an unbiased randomness $\xi_{t,s}$ and a biased non-random approximation error $\eta_{t,s}$:
\[
    \rmu_{t,s} = \mmu_{t,s} + \eta_{t,s} + \xi_{t,s}.
\]
We bound $\eta$ and $\xi$ separately.

Notice that $\beta_t$ is a $|S| \times |A|$ right stochastic matrix for every $t$. Similarly, $P_{s}$ is also a right stochastic matrix for every $s \in S$. Let us define the $|S|\times|S|$ matrix $M_t$ as $M_{t,s,s'} = (\sum_{a \in A} \beta_{t,s}^a P_{s,s'}^a)_{s,s' \in S}$. $M_t$ is also a right stochastic matrix for every $t$ because $\sum_{s'} M_{t,s,s'} = \sum_{s'} \sum_{a \in A} \beta_{t,s}^a P_{s,s'}^a = \sum_{a \in A} \beta_{t,s}^a \sum_{s'} P_{s,s'}^a = \sum_{a \in A} \beta_{t,s}^a = 1$.

% Let us now derive some inequalities that will be useful in our proof. 
Given $\rmu_t$ and $\beta_t$, $\ralpha_t$ is computed using the rounding function in Lemma~\ref{lm:round} as: $\ralpha_{t,s} = \round(\rmu_{t,s} \beta_{t,s})$. As per the properties of the rounding function, $\ralpha_{t,s}^a \in \{ \lfloor \rmu_{t,s} \beta_{t,s}^a \rfloor, \lceil \rmu_{t,s} \beta_{t,s}^a \rceil \} \implies \rmu_{t,s} \beta_{t,s}^a - 1 \le \ralpha_{t,s}^a \le \rmu_{t,s} \beta_{t,s}^a + 1$.

Let us first bound the bias term $\eta_{t,s}$ caused by the approximation error due to rounding. 
\MJnote{should it be $\eta$ below or $n_t$?}
\begin{lemma}
$-(t-1)|S||A| \le n_t \le (t-1)|S||A|$.
\end{lemma}
\begin{proof}
At time $t=1$, $\rmu_1 = \mmu_1 = \mu_1$, so $\eta_{1,s_1} = 0$ for every $s_1 \in S$.

At time $t=2$, the mean-field state $\mmu_2$ is deterministic and is given by $\mmu_{2,s_2} = \sum_{s_1 \in S, a_1 \in A} \mu_{1,s_1} \beta_{1,s_1}^{a_1} P_{s_1,s_2}^{a_1} = \sum_{s_1} \mu_{1,s_1} \sum_{a_1} \beta_{1,s_1}^{a_1} P_{s_1,s_2}^{a_1} \implies \mmu_2^\intercal = \mu_1^\intercal M_1$. 
On the other hand, for the real-life process, first, the action $\ralpha_1$ is computed based on $\mu_1$ and $\beta_1$ by rounding, then $\rmu_{2,s_2} = \sum_{s_1, a_1} \sum_{\ell \in [\ralpha_{1,s_1}^{a_1}]} \b1{\{x_{s_1,\ell}^{a_1} = s_2\}}$ where $x_{s_1,\ell}^{a_1} \sim P_{s_1}^{a_1}$.
\begin{align*}
    \Exp[\rmu_{2,s_2}] &= \Exp_{x_{s_1,\ell}^{a_1} \sim P_{s_1}^{a_1}}\left[\sum_{s_1, a_1} \sum_{\ell \in [\ralpha_{1,s_1}^{a_1}]} \b1{\{x_{s_1,\ell}^{a_1} = s_2\}}\right] \\
    &= \sum_{s_1, a_1} \alpha_{1,s_1}^{a_1} P_{s_1,s_2}^{a_1} \le \sum_{s_1, a_1} (\mu_{1,s_1} \beta_{1,s_1}^{a_1} + 1) P_{s_1,s_2}^{a_1},
\end{align*}
because $\alpha_{1,s_1}^{a_1} \le \mu_{1,s_1} \beta_{1,s_1}^{a_1} + 1$. Putting in a vector form, $\Exp[\rmu_2^\intercal] \le \mu_1^\intercal M_1 + q^\intercal = \mmu_2^\intercal + q^\intercal$, where $q = (\sum_{s,a} P_{s,s'}^{a})_{s' \in S}$. In a similar manner, using $\alpha_{1,s_1}^{a_1} \ge \mu_{1,s_1} \beta_{1,s_1}^{a_1} - 1$, we get $\Exp[\rmu_2^\intercal] \ge \mu_1^\intercal M_1 - q^\intercal$. Computing $\eta_2 = \Exp[\rmu_2] - \mmu_2$ we get
\begin{align*}
    -q \le \eta_2 \le q.
\end{align*}

At time $t$, following similar steps as before, we get the mean-field state 
\[
    \mmu_t^\intercal = \mmu_{t-1}^\intercal M_{t-1} = \mmu_{t-2}^\intercal M_{t-2} M_{t-1} = \ldots = \mu_1^\intercal \prod_{\ell = 1}^{t-1} M_{\ell}.
\]
Now, for the real-life state $\rmu_t$, we have
\begin{align*}
    \Exp[\rmu_t] &= \Exp\left[\left(\sum_{s, a} \alpha_{t-1,s}^{a} P_{s,s'}^{a}\right)_{s' \in S}\right] \\
    &\le \Exp\left[ \left(\sum_{s, a} (\mu_{t-1,s} \beta_{t-1,s}^{a} + 1) P_{s,s'}^{a}\right)_{s' \in S} \right] \\
    \implies \Exp[\rmu_t^\intercal] &\le \Exp\left[ \rmu_{t-1}^\intercal M_{t-1} + q^\intercal \right] = \Exp\left[ \rmu_{t-1}^\intercal \right] M_{t-1} + q^\intercal \\
    &\le (\Exp\left[ \rmu_{t-2}^\intercal \right] M_{t-2} + q^\intercal) M_{t-1} + q^\intercal \\
    &\le ((\Exp\left[ \rmu_{t-3}^\intercal \right] M_{t-3} + q^\intercal) M_{t-2} + q^\intercal) M_{t-1} + q^\intercal \\
    &\le \ldots \le \mu_1^\intercal \prod_{\ell = 1}^{t-1} M_{\ell} + \sum_{k = 2}^{t-1} q^\intercal \prod_{\ell = k}^{t-1} M_{\ell} + q^\intercal \\
    &= \mmu_t^\intercal + \sum_{k = 2}^{t-1} q^\intercal \prod_{\ell = k}^{t-1} M_{\ell} + q^\intercal.
\end{align*}
In a similar manner, we can lower bound $\Exp[\rmu_t]$ as
\[
    \Exp[\rmu_t^\intercal] \ge \mmu_t^\intercal - \sum_{k = 2}^{t-1} q^\intercal \prod_{\ell = k}^{t-1} M_{\ell} - q^\intercal.
\]
As the matrix $M_t$ is right stochastic for every $t$, then so is $\prod_{\ell = k}^{t} M_{\ell}$ for every $k \in [t]$ and $t \in [H]$. Therefore, $||q^\intercal \prod_{\ell = k}^{t} M_{\ell} ||_1 = ||q^\intercal||_1$ for every $k \le t$. Now, for every $s \in S$, $q_s \le ||q||_1 = \sum_{s',a,s''} P_{s',s''}^{a} = |S||A|$. Putting everything together, we have
\[
     -(t-1)|S||A| \le n_t \le (t-1)|S||A|.
\]
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The following was the longer analysis by decomposing each time-step 
%% into N steps.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As tools for analysis, we shall (1) tag each of the $N$ beneficiaries and track their transitions and (2) decompose each time-step into $N$ time-sub-steps.
\begin{enumerate}
    \item Let the beneficiaries be indexed by $j = 1, 2, \ldots, N$ in an arbitrary but fixed order. Let $X_{t,j}$ be a random variable representing the one-hot representation of the state of beneficiary $j$ at time $t$. Notice that $\rmu_t = \sum_{j \in [N]} X_{t,j}$ by definition. Also note that $X_{1,j}$ is given to us (or we can compute it from $\mu_1$ by arbitrarily assigning each beneficiary to a state while maintaining $\mu_1 = \sum_{j \in [N]} X_{1,j}$).
    \item We shall denote a time-sub-point in the sequence of time-sub-steps by a pair $(t,j)$ where $t \in [H]$ and $j \in [N]$. The sequence of time-sub-steps follow $(t,j) \rightarrow (t,j+1)$ if $j < N$ and $(t,N) \rightarrow (t+1,1)$ otherwise. We shall denote $(t,N+1) \equiv (t+1,1)$. Between time-sub-point $(t,j)$ and $(t,j+1)$, only beneficiary $j$ makes a transition, and in particular their $t$-th transition, everyone else remain in their current states.
\end{enumerate}

Let $(\cF_{\tau})_{\tau \in \Tau}$ denote the filtration where $\cF_{\tau}$ models the information available at time-sub-point $\tau$. 

Let us focus our attention to the time-sub-point $(t,1)$. When we reach this time-sub-point, all the beneficiaries have made exactly $(t-1)$ transitions, and we know the realization of $X_{t,j}$ and $\rmu_t$. Formally, $X_{t,j}$ and $\rmu_t$ are $\cF_{t,1}$-measurable and $\Exp[X_{t,j} \mid \cF_{t,1}] = X_{t,j}$ and $\Exp[\rmu_t \mid \cF_{t,1}] = \rmu_t$. As we deterministically know $\rmu_t$, we can deterministically compute $\ralpha_{t,s}^a = \beta_{t,s}^a \rmu_{t,s}$. Also, note that there must be exactly $\rmu_{t,s}$ beneficiaries $j \in [N]$ with $X_{t,j} = e_s$, where $e_s$ is the standard basis vector of length $|S|$. Then, we arbitrarily but deterministically assign $\ralpha_{t,s}^a$ beneficiaries out of these $\rmu_{t,s}$ beneficiaries in state $s$ to action $a$ (e.g., in lexicographic order). By following this procedure, let us say that beneficiary $j$ was assigned action $a_{t,j}$. Then, at time $t+1$, we know that the state of beneficiary $j$ has the distribution $P_{s_{t,j}}^{a_{t,j}}$, where $s_{t,j} = \arg \max_{s} X_{t,j}$, i.e., $s_{t+1,j} \sim P_{s_{t,j}}^{a_{t,j}}$ and $X_{t+1,j}$ is the one-hot representation of $s_{t+1,j}$. This also tells us that $\Exp[X_{t+1,j} \mid \cF_{t,1}] = P_{s_{t,j}}^{a_{t,j}}$. As the beneficiary $j$ does its transition (just) after time $(t,j)$, we can also write $\Exp[X_{t+1,j} \mid \cF_{t,j}] = P_{s_{t,j}}^{a_{t,j}}$, and also $\Exp[X_{t+1,j} \mid \cF_{t,j+1}] = X_{t+1,j}$ because $X_{t+1,j}$ is $\cF_{t,j+1}$ measurable.

Now, notice that $-1 \le X_{t+1,j} - P_{s_{t,j}}^{a_{t,j}} \le 1$ almost surely because each for each $s \in S$, $0 \le X_{t+1,j,s} \le 1$ and $0 \le P_{s_{t,j},s}^{a_{t,j}} \le 1$. Using this, we claim that for any 

Let us denote this sequence of time-sub-steps as $\Tau = ((1,1), (1,2),$ $\ldots, (t,j), (t,j+1), \ldots, (H,N), (H+1,1))$ and an element of $\Tau$ as $\tau = (t,j)$. Given, $\tau = (t,j)$, we use notation: $\tau+1 = (t,j+1)$. For $\tau \ge (1,N)$, let us define $Y_{\tau}$ as: $Y_{\tau} = X_{\tau-1+N} - P_{s_{\tau-1}}^{a_{\tau-1}}$. Based on the discussion in the previous paragraph, given $\tau = (t,j)$, $\Exp[X_{t+1,j} \mid \cF_{t,j}] = P_{s_{t,j}}^{a_{t,j}} \implies \Exp[X_{\tau + N} \mid \cF_{\tau}] = P_{s_{\tau}}^{a_{\tau}} \implies \Exp[Y_{\tau + 1} \mid \cF_{\tau}] = 0$. Also, as $X_{t+1,j}$ is $\cF_{t,j+1}$  measurable, i.e., $X_{\tau + N}$ is $\cF_{\tau+1}$-measurable, so $Y_{\tau+1}$ is $\cF_{\tau+1}$-measurable. Now, further notice that $||Y_{\tau+1}||_{\infty} = ||Y_{t,j+1}||_{\infty} = ||X_{t+1,j} - P_{s_{t,j}}^{a_{t,j}}||_{\infty} \le 1$ almost surely. Putting it together, we have for $\tau \ge (1,N)$, $Y_{\tau}$ satisfies
\begin{enumerate}
    \item Martingale difference property: $Y_{\tau}$ is $\cF_{\tau}$ measurable and $\Exp[Y_{\tau} \mid \cF_{\tau-1}] = 0$.
    \item Predictable bounds: $0 \le Y_{\tau} \le 1$ almost surely.
\end{enumerate}


(i) $Y_{\tau}$ is $\cF_{\tau}$-measurable for every $\tau$, and (ii) $\Exp[Y_{\tau + 1} \mid \cF_{\tau}] = 0$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Additional old stuff related to bounds using Azuma--Hoeffding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Now, let $Y_{s, \ell}^a(Q)^\intercal = (Z_{s, \ell}^a - P_{s}^a)^\intercal Q$ for an arbitrary right stochastic matrix $Q$. Notice that $\Exp[Y_{s, \ell}^a(Q)^\intercal \mid \cF_t] = (\Exp[{Z_{s, \ell}^a} \mid \cF_t] {P_{s}^a})^\intercal Q = 0$. Also notice that $-1 \le ||Y_{s, \ell}^a(Q)||_{\infty} \le 1$ because 


$0 \le ||Z_{s, \ell}^a||_{\infty}, ||P_{s}^a||_{\infty} \le 1$, and $-1 \le ||Y_{s, \ell}^a||_1 \le 1$ because $||Z_{s, \ell}^a||_1 = ||P_{s}^a||_1 = 1$. Also observe that $X_{t+1} = \sum_{s, a} \sum_{\ell \in [\ralpha_{t,s}^a]} Y_{s,\ell}^a $.

As the random variables $Y_{s, \ell}^a$ are all bounded, applying Hoeffding lemma (\cite{van2014probability}, Lemma~3.6) we get $\Exp[e^{\lambda Y_{s, \ell}^a}] \le e^{-\lambda^2/2}$, i.e., $Y_{s, \ell}^a$ is $1$-subgaussian. Further, as the random variables $Y_{s, \ell}^a$ are all independent given $\cF_t$, have mean $\Exp[Y_{s, \ell}^a \mid \cF_t] = 0$, and are $1$-subgaussian, applying Azuma-Hoeffding inequality (\cite{van2014probability}, Lemma~3.7) to $X_{t+1} = \sum_{s, a} \sum_{\ell \in [\ralpha_{t,s}^a]} Y_{s,\ell}^a $, we get 
\[
    \Exp[e^{\lambda X_{t+1}}] \le e^{-\lambda^2 N^2 /2},
\]
i.e., $X_{t+1}$ is $N$-subgaussian. Further, as shown earlier, $X_{t+1}$ satisfies martingale difference property



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Unsuccessful attempt to prove MF randomnes error doesn't depend upon K
%% Got stuck while solving for this.. given probability distributions
%% x, y, u, v in n-dim find a matrix A that is column stochastic such that
%% Ax = y and Bu = v. We found counterexample for size n=2.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Similar Reward Functions across Clusters}
Most of the application domains for RMABs have homogeneous rewards functions across all arms, i.e., $R_{t,i,s}^a = R_{t,i',s}^a$ for every $i,i' \in [K]$ and for every  $t$, $s$, and $a$. If a given RMAB satisfies this condition, or an approximate version of this condition of the form $R_{t,i,s}^a \le \eta R_{t,i',s}^a$ for every $i,i' \in [K]$, for some constant $\eta$, and for every $t,s,a$, then we can bound the error between mean-field and optimal expected reward by a factor proportional to $\sqrt{K}$ (TODO) if we use bucket sampling. Even if the rewards are not exactly homogeneous, the approximate version of homogeneity may be easy to satisfy by introducing a small number of additional states. In the next section, we shall look at the general case with no assumptions about the reward function $R$, and provide an error bound proportional to $K$ (TODO).

\begin{lemma}\label{lm:stateBoundH}
For every $1 \le t \le T-1$, when the mean-field algorithm uses bucket sampling,
\begin{align*}
    \Prob[ \sum_i(\rmu_{t+1,i} - \mmu_{t+1,i}) \ge t|S|\epsilon ] &\le t|S| \exp{ \left(- \frac{\epsilon^2}{2(N+K|S||A|^2)} \right)}, \\
    \Prob[ \sum_i(\rmu_{t+1,i} - \mmu_{t+1,i}) \le - t|S|\epsilon ] &\le t|S| \exp{ \left(- \frac{\epsilon^2}{2(N+K|S||A|^2)} \right)}.
\end{align*}
\end{lemma}
\begin{proof}
Notice that $\beta_{t,i}$ is an $|S| \times |A|$ right stochastic matrix for every $t$ and $i$. Similarly, $P_{t,i,s}$ is also a right stochastic matrix for every $t,i,s$. Let us define the $|S|\times|S|$ matrix $M_{t,i}$ as $M_{t,i,s,s'} = \sum_{a \in A} \beta_{t,i,s}^a P_{t,i,s,s'}^a$. $M_{t,i}$ is also a right stochastic matrix for every $t$ and $i$ because $\sum_{s'} M_{t,i,s,s'} = \sum_{s'} \sum_{a \in A} \beta_{t,i,s}^a P_{t,i,s,s'}^a = \sum_{a \in A} \beta_{t,i,s}^a \sum_{s'} P_{t,i,s,s'}^a = \sum_{a \in A} \beta_{t,i,s}^a = 1$.

At the initial time-point $t=1$, the real-life state and the mean-field state are both equal to $\mu_1$: $\rmu_1 = \mmu_1 = \mu_1$. At time $t$, there are two sources of divergence (error) between the mean-field state $\mmu_{t}$ and the real-life state $\rmu_{t}$:
\begin{enumerate}
    \item Rounding. For each $t$, we do rounding to compute the real-life action $\ralpha_{t,i,s} = \round(\beta_{t,i,s} \rmu_{t,i,s})$, but not for the mean-field action $\malpha_{t,i,s} = \beta_{t,i,s} \mmu_{t,i,s}$. 
    % Notice that the rounding error may add bias.
    \item Randomness. The real-life state $\rmu_{t+1}$ is a random function of $\ralpha_t$ because of the stochasticity of the transitions.
\end{enumerate}
As mentioned, due to rounding, $\ralpha_{t,i,s}^a$ may not be equal to $\beta_{t,i,s}^a \rmu_{t,i,s}$. Let us define $\rbeta_{t,i,s}^a = \ralpha_{t,i,s}^a / \rmu_{t,i,s}$ if $\rmu_{t,i,s} > 0$ and $\rbeta_{t,i,s}^a = \beta_{t,i,s}^a$ otherwise. As we had defined the right stochastic matrix $M_{t,i}$ based on $\beta_{t,i}$ and $P_{t,i}$, we similarly define the $|S|\times|S|$ right stochastic matrix $\rM_{t,i} = (\sum_a \beta_{t,i,s}^a P_{t,i,s,s'}^a)_{s,s' \in S}$ based on $\rbeta_{t,i}$ and $P_{t,i}$.

Let $(\cF_{t})_{t \in [T]}$ denote the natural filtration with respect to $\rmu_t$, i.e., $\cF_{t}$ models the information available at time $t$. Notice that $\rmu_t$ is $\cF_t$-measurable by definition. 

In the next segment of the proof, we will try to measure how much \textit{new} error is introduced between the mean-field estimate and the real-life process in a given time step due to rounding and randomness. Later in the proof, we shall  quantify how this error gets accumulated over time. 

\textbf{Let us focus on a particular time-step $t \rightarrow (t+1)$.} 
At time $t$, we know the realization of $\rmu_t$. Given $\rmu_t$, we know that $\beta_t$ is deterministic as per its definition, and we also know that the action $\ralpha_{t,i,s} = \round(\beta_{t,i,s} \rmu_{t,i,s})$ is also deterministic because the rounding function and all the inputs to it are deterministic. 
Remember that $\ralpha_{t,i,s}^a$ is a non-negative integer and denotes the number of arms in cluster $i$ state $s$ at time $t$ for which we play action $a$. Also note that $\sum_{i,s,a} \ralpha_{t,i,s}^a = \sum_{i,s} \rmu_{t,i,s} = \sum_i N_i = N$ for every $t$.

Given $\rmu_t$, $\rmu_{t+1}$ is a random variable given by \\
$\rmu_{t+1,i,s'} = \sum_{s, a} \sum_{\ell \in [\ralpha_{t,i,s}^a]} \bI{\{z_{\ell,i,s}^a = s'\}}$ where $z_{\ell,i,s}^a \sim P_{t,i,s}^a$. To simplify notation for the upcoming analysis, let us index the $N$ arms by $j = 1, 2, \ldots, N$ and denote arm $j$'s cluster, state, and action at time $t$ by $i_j$, $s_j$, and $a_j$. Let $\cN_i = \{ j \mid i_j = i\}$. Notice that, by definition, exactly $\ralpha_{t,i,s}^a$ arms will have cluster, state, and action equal to $i$, $s$ and $a$, respectively, i.e., $\sum_j \bI{\{i_j = i\}} \bI{\{s_j = s\}} \bI{\{a_j = a\}} = \ralpha_{t,i,s}^a$. 

Let $Z_j$ be the one-hot random variable that denotes the state of arm $j$ at time $t+1$; so, $(\arg\max_{s} Z_{j,s}) \sim P_{t,i_j,s_j}^{a_j}$. Notice that $Z_j$ for arm $j$ is picked independently of the other arms given $\rmu_t$. We can rewrite $\rmu_{t+1}$ as $\rmu_{t+1,i} = \sum_{j \in \cN_i} Z_j$. Further, $\Exp[\rmu_{t+1,i} \mid \cF_t]$ is 
\begin{multline*}
    \Exp[\rmu_{t+1,i} \mid \cF_t] = \Exp \left[ \left. \sum_{j \in \cN_i} Z_j \right| \cF_t \right] = \sum_{j \in \cN_i} \Exp [  Z_j \mid \cF_t ] \\
    = \sum_{j \in \cN_i} P_{t,i,s_j}^{a_j} = \sum_{s, a} \ralpha_{t,i,s}^a P_{t,i,s}^a = \sum_{s} \rmu_{t,i,s} \sum_a \rbeta_{t,i,s}^a P_{t,i,s}^a = \rM_{t,i}^\intercal \rmu_{t,i} .
\end{multline*}
On the other hand, given $\rmu_{t}$, if we were to estimate the expected value of the state at time $t+1$ without rounding, as done by the mean-field algorithm, then estimate of $\rmu_{t+1,i}$ would have been $\sum_{s,a} \rmu_{t,i,s} \beta_{t,i,s}^a P_{t,i,s}^a = M_{t,i}^\intercal \rmu_{t,i} $. So, the newly introduced rounding error in this transition between the real-life state and the mean-field estimated state, for cluster $i$, is
\[
    \rM_{t,i}^\intercal \rmu_{t,i} - M_{t,i}^\intercal \rmu_{t,i}.
\]
Let us provide an \textit{almost surely} bound for this error. As per our construction of the rounding function, we know that
\begin{multline}\label{eq:lm:stateError:1}
    \ralpha_{t,i,s}^a \in \{ \lfloor \rmu_{t,i,s} \beta_{t,i,s}^a \rfloor, \lceil \rmu_{t,i,s} \beta_{t,i,s}^a \rceil \} \\
    \implies - 1 \le \ralpha_{t,i,s}^a - \rmu_{t,i,s} \beta_{t,i,s}^a \le  + 1 \\
    \implies - \sum_{s, a} P_{t,i,s}^a \le \sum_{s, a} (\ralpha_{t,i,s}^a - \rmu_{t,i,s} \beta_{t,i,s}^a) P_{t,i,s}^a \le  \sum_{s, a}  P_{t,i,s}^a \\
    \implies -q_{t,i} \le \rM_{t,i}^\intercal \rmu_{t,i} - M_{t,i}^\intercal \rmu_{t,i} \le q_{t,i},
\end{multline}
where $q_{t,i}$ is the $|S|$-dimensional vector defined as $q_{t,i,s'} = \sum_{s, a}  P_{t,i,s,s'}^a$. 
% Adding the error in \eqref{eq:lm:stateError:roundBound2} across all clusters, we get
% \begin{equation}
%     -\sum_{i} q_i \le \sum_i \rM_{t,i}^\intercal \rmu_{t,i} - \sum_i M_{t,i}^\intercal \rmu_{t,i} \le \sum_i q_i.
% \end{equation}

Next, let us focus on the divergence between $\rmu_{t+1,i}$ and  $\Exp[\rmu_{t+1,i} \mid \cF_t] = \rM_{t,i}^\intercal \rmu_{t,i}$. We shall show that $\rmu_{t+1,i}$ is close to $\rM_{t,i}^\intercal \rmu_{t,i}$ with high probability.

Given $\mu_t$, for each arm $j$, $Z_j$ is sampled independently. Also note that $0 \le Z_{j,s} \le 1$ for every $s$. Applying Hoeffding's inequality (Lemma~\ref{lm:hoeffding}) for each $s \in S$ we have
\begin{equation*}
    \Prob \left[ \sum_j Z_{j,s} - \sum_{i} (\rM_{t,i}^\intercal \rmu_{t,i})_s \ge \epsilon \right] \le \exp{ \left(- \frac{2\epsilon^2}{N} \right)}.
\end{equation*}
Applying union bound for every $s \in S$, we get
\begin{equation}\label{eq:lm:stateError:2}
    \Prob \left[ \sum_j Z_j - \sum_{i} \rM_{t,i}^\intercal \rmu_{t,i} \ge_{any} \epsilon \right] \le |S|\exp{ \left(- \frac{2\epsilon^2}{N} \right)}.
\end{equation}
We know that $\sum_{j \in \cN_i} Z_j = \rmu_{t+1,i}$, so $\sum_j Z_j = \sum_i \rmu_{t+1,i}$. Combining \eqref{eq:lm:stateError:1} for each $i$ with \eqref{eq:lm:stateError:2}, we have
\begin{equation}\label{eq:lm:stateError:3}
    \Prob \left[ \sum_i \rmu_{t+1,i} - \sum_{i} M_{t,i}^\intercal \rmu_{t,i} \ge_{any} \epsilon + q_t \right] \le |S|\exp{ \left(- \frac{2\epsilon^2}{N} \right)},
\end{equation}
where $q_t = \sum_i q_{t,i}$. For every $t$, let $\nu_t = \sum_i \rmu_{t,i}$. For every $t$, let us also define the $|S|\times|S|$ matrix $Q_t$, where the $s$-th row of $Q_t$ is defined as $Q_{t,s} = \frac{\sum_i \rmu_{t,i,s} M_{t,i,s}}{ \sum_i \rmu_{t,i,s}}$, where $M_{t,i,s}$ is the $s$-th row of $M_{t,i}$. Notice that by definition, $\sum_{i} M_{t,i}^\intercal \rmu_{t,i} = Q_t^\intercal (\sum_i \rmu_{t,i,s}) = Q_t^\intercal \nu_t$. Leveraging this newly introduced notation, we can rewrite our bound in \eqref{eq:lm:stateError:3} as
\begin{equation}\label{eq:lm:stateError:4}
    \Prob \left[ \nu_{t+1} - Q_t^\intercal \nu_t \ge_{any} \epsilon + q_t \right] \le |S|\exp{ \left(- \frac{2\epsilon^2}{N} \right)}.
\end{equation}





The bound in \eqref{eq:lm:stateError:4} is true for all $t \ge 1$. Let us pick a time $\tau \le t$. If $\nu_{\tau+1} - Q_{\tau}^\intercal \nu_{\tau} \le_{all} q_{\tau} + \epsilon$, then multiplying both sides by $\left(\prod_{\ell = \tau+1}^{t} Q_{\ell} \right)^\intercal$ we have
\begin{equation}\label{eq:lm:stateError:5}
    \left(\prod_{\ell = \tau+1}^{t} Q_{\ell} \right)^\intercal \nu_{\tau+1} - \left(\prod_{\ell = \tau}^{t} Q_{\ell} \right)^\intercal \nu_{\tau} \le_{all} \left(\prod_{\ell = \tau+1}^{t} Q_{\ell} \right)^\intercal (q_{\tau} + \b1 \epsilon ),
\end{equation}
where $\b1$ is the vector of all ones. Let us denote the matrix $\prod_{\ell = \tau}^{t} Q_{\ell}$ as $Q_{\tau:t}$. As $Q_{\ell}$ is right stochastic for every $\ell$, $Q_{\tau:t}$ is also right stochastic. Combining equations \eqref{eq:lm:stateError:4} and \eqref{eq:lm:stateError:5} for $\tau = 1, \ldots, t$ and applying union-bound we get
\begin{multline*}
    \Prob \left[ \sum_{\tau = 1}^{t} (Q_{\tau+1:t}^\intercal \nu_{\tau+1} - Q_{\tau:t}^\intercal \nu_{\tau}) \ge_{any} \sum_{\tau = 1}^{t}  Q_{\tau+1:t}^\intercal (q_{\tau} + \b1 \epsilon ) \right] \\
    \le t |S| \exp{ \left(- \frac{\epsilon^2}{2N} \right)}.
\end{multline*}
Notice that sum $\sum_{\tau = 1}^{t} (Q_{\tau+1:t}^\intercal \nu_{\tau+1} - Q_{\tau:t}^\intercal \nu_{\tau})$ is telescoping and is equal to $\nu_{t+1} - Q_{1:t}^\intercal \nu_1$. Notice that $\nu_1 = \sum_i \rmu_{1,i} = \sum_i \mu_{1,i} = \sum_i \mmu_{1,i}$, and by definition, $Q_{1:t}^\intercal \mmu_1 = \mmu_{t+1}$. So, we get 
\begin{equation}\label{eq:lm:stateError:boundt3}
    \Prob \left[ \nu_{t+1} - \mmu_{t+1} \ge \sum_{\tau = 1}^{t}  Q_{\tau+1:t}^\intercal (q + \b1 \epsilon ) \right] \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)}.
\end{equation}
Let us now try to bound the error term: $\sum_{\tau = 1}^{t}  Q_{\tau+1:t}^\intercal (q + \b1 \epsilon )$. As $Q_{\tau+1:t}$ is right stochastic, every element of the matrix is $\le 1$, and therefore, $Q_{\tau+1:t}^\intercal q \le \sum_{s'} q_{s'} = \sum_{s,a,s'} P_{t,s,s'}^a = |S||A|$ and $Q_{\tau+1:t}^\intercal \b1 \epsilon \le \epsilon |S| $. Putting it back to \eqref{eq:lm:stateError:boundt3} we get
\begin{equation}\label{eq:lm:stateError:boundt4}
    \Prob[ \nu_{t+1} - \mmu_{t+1} \ge t|S|(|A| + \epsilon) ] \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)},
\end{equation}
for every $1 \le t \le T-1$ and $\epsilon > 0$. Following analogous steps, we get
\begin{equation}\label{eq:lm:stateError:boundt5}
    \Prob[ \nu_{t+1} - \mmu_{t+1} \le - t|S|(|A| + \epsilon) ] \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)},
\end{equation}
for every $1 \le t \le T-1$ and $\epsilon > 0$.


The bound in \eqref{eq:lm:stateError:boundt1} is true for all $t \ge 1$. Now, pick a time $\tau \le t$. If $\rmu_{\tau+1} - M_{\tau}^\intercal \rmu_{\tau} < q + \epsilon$, 
% or equivalently $\rmu_{\tau+1}^\intercal - \rmu_{\tau}^\intercal M_{\tau} < q^\intercal + \epsilon \b1^\intercal$, where $\b1$ is the vector of all ones, 
then multiplying both sides by $\left(\prod_{\ell = \tau+1}^{t} M_{\ell} \right)^\intercal$ we have
\begin{equation}\label{eq:lm:stateError:boundt2}
    \left(\prod_{\ell = \tau+1}^{t} M_{\ell} \right)^\intercal \rmu_{\tau+1} - \left(\prod_{\ell = \tau}^{t} M_{\ell} \right)^\intercal \rmu_{\tau} < \left(\prod_{\ell = \tau+1}^{t} M_{\ell} \right)^\intercal (q + \b1 \epsilon ),
\end{equation}
where $\b1$ is the vector of all ones. Let us denote the matrix $\prod_{\ell = \tau}^{t} M_{\ell}$ as $M_{\tau:t}$. As $M_{\ell}$ is right stochastic for every $\ell$, $M_{\tau:t}$ is also right stochastic. Combining equations \eqref{eq:lm:stateError:boundt1} and \eqref{eq:lm:stateError:boundt2} for $\tau = 1, \ldots, t$ and applying union-bound we get
\begin{multline*}
    \Prob \left[ \sum_{\tau = 1}^{t} (M_{\tau+1:t}^\intercal \rmu_{\tau+1} - M_{\tau:t}^\intercal \rmu_{\tau}) \ge \sum_{\tau = 1}^{t}  M_{\tau+1:t}^\intercal (q + \b1 \epsilon ) \right] \\
    \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)}.
\end{multline*}
Notice that sum $\sum_{\tau = 1}^{t} (M_{\tau+1:t}^\intercal \rmu_{\tau+1} - M_{\tau:t}^\intercal \rmu_{\tau})$ is telescoping and is equal to $\rmu_{t+1} - M_{1:t}^\intercal \rmu_1$. Notice that $\rmu_1 = \mu_1 = \mmu_1$, and by definition, $M_{1:t}^\intercal \mmu_1 = \mmu_{t+1}$. So, we get 
\begin{equation}\label{eq:lm:stateError:boundt3}
    \Prob \left[ \rmu_{t+1} - \mmu_{t+1} \ge \sum_{\tau = 1}^{t}  M_{\tau+1:t}^\intercal (q + \b1 \epsilon ) \right] \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)}.
\end{equation}
Let us now try to bound the error term: $\sum_{\tau = 1}^{t}  M_{\tau+1:t}^\intercal (q + \b1 \epsilon )$. As $M_{\tau+1:t}$ is right stochastic, every element of the matrix is $\le 1$, and therefore, $M_{\tau+1:t}^\intercal q \le \sum_{s'} q_{s'} = \sum_{s,a,s'} P_{t,s,s'}^a = |S||A|$ and $M_{\tau+1:t}^\intercal \b1 \epsilon \le \epsilon |S| $. Putting it back to \eqref{eq:lm:stateError:boundt3} we get
\begin{equation}\label{eq:lm:stateError:boundt4}
    \Prob[ \rmu_{t+1} - \mmu_{t+1} \ge t|S|(|A| + \epsilon) ] \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)},
\end{equation}
for every $1 \le t \le T-1$ and $\epsilon > 0$. Following analogous steps, we get
\begin{equation}\label{eq:lm:stateError:boundt5}
    \Prob[ \rmu_{t+1} - \mmu_{t+1} \le - t|S|(|A| + \epsilon) ] \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)},
\end{equation}
for every $1 \le t \le T-1$ and $\epsilon > 0$.
\end{proof}


Let us now reintroduce the notation for clusters (move back to our original notation) and extend the proof of Lemma~\ref{lm:stateError} to an RMAB with $K$ clusters.
\begin{proof}[Proof of Lemma~\ref{lm:stateError} with $K$ clusters]
Let us convert our original RMAB with clusters to a larger RMAB without clusters (or with only one cluster). In the new RMAB, the state of an arm is not an element of $S$ but rather an element $i!s$ of $S' = [K] \times S$; we shall use this notation $i!s$, which is equivalent to $(i,s) \in [K] \times S$, but will help us avoid confusion. We shall specify the other parameters of the new RMAB suitably to simulate the behavior the old RMAB. All the arms have a homogeneous transition function $P'$, where $P_{t,i!s,i'!s'}^{'a} = P_{t,s,s'}^a$ if $i = i'$ and $0$ otherwise. This transition matrix ensures that if an arm starts in cluster $i$, then they always remain in cluster $i$. In a similar fashion, we can convert the old normalized action $\beta$ to the new format as $\beta_{t,i!s}^{'a} = \beta_{t,i,s}^a$. Everything else can be converted similarly, e.g., the real-life state $\rmu_{t}$ at time $t$ can be written as $\rmu'_{t,i!s} = \rmu_{t,i,s}$, etc. We shall denote the parameters of the new RMAB using a `prime', like $S'$, $P'$, $\rmu'$, $\mmu'$, etc.

Let us define $M_t'$ in the same way we had defined $M_t$ in the proof for only one cluster:  $M_{t,i!s,i'!s'} = \sum_{a \in A} \beta_{t,i!s}^{'a} P_{t,i!s,i'!s'}^{'a}$. Notice that $M_t$ is a block-diagonal matrix of size $K|S| \times K|S|$, where the $i$-th block in the diagonal of $M'_t$ is of size $|S|\times|S|$ and is equal to $(\sum_{a \in A} \beta_{t,i,s}^{a} P_{t,i,s,s'}^{a})_{s,s' \in S}$. All the off-diagonal blocks are equal to $0$ because $P_{t,i!s,i'!s'}^{'a} = 0$ if $i \neq i'$.

Now, the reader can check that the proof provided for a single cluster applies directly to this new RMAB. But, the reader may notice that the final bound that we would get from \eqref{eq:lm:stateError:boundt4} and \eqref{eq:lm:stateError:boundt5} is looser than what we have claimed in our lemma statement. In particular, consider the bound in \eqref{eq:lm:stateError:boundt4}. If we put the parameters of our new RMAB into this inequality, we get
\begin{equation}
    \Prob[ \rmu'_{t+1} - \mmu'_{t+1} \ge t|S'|(|A| + \epsilon) ] \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)},
\end{equation}
which is not as tight as required because $|S'| = K|S|$. To fix this issue, let us take a step back and write inequality \eqref{eq:lm:stateError:boundt3} for our current RMAB
\begin{equation}\label{eq:lm:stateError:boundt6}
    \Prob \left[ \rmu'_{t+1} - \mmu'_{t+1} \ge \sum_{\tau = 1}^{t}  M_{\tau+1:t}^{'\intercal} (q' + \b1 \epsilon ) \right] \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)}.
\end{equation}
Notice that $M'_{\ell}$ is a block-diagonal right stochastic matrix of size $K|S|\times K|S|$, where the blocks are of size $|S|\times|S|$ each, and there are $K$ of them. Therefore, the matrix $M'_{\tau+1:t}$, which is the product of $t-\tau$ of such block-diagonal right stochastic matrices, is also block-diagonal and right stochastic. 

Now, let us now try to bound the error term: $\sum_{\tau = 1}^{t}  M_{\tau+1:t}^{'\intercal} (q' + \b1 \epsilon )$. As $M'_{\tau+1:t}$ is right stochastic, every element of the matrix is $\le 1$. Further, as $M'_{\tau+1:t}$ is block diagonal and of the form discussed earlier, in the column $i!s$ of $M'_{\tau+1:t}$, only the elements in rows $i!1$ to $i!|S|$ can be positive. Therefore, $(M_{\tau+1:t}^\intercal \b1)_{i|s} = \sum_{i'|s'} (M'_{\tau+1:t})_{i'!s',i!s} = \sum_{s'} (M'_{\tau+1:t})_{i!s',i!s} \le |S|$. Similarly, the $i!s''$-th element of $M_{\tau+1:t}^{'\intercal} q'$ is bounded by
\begin{multline*}
    (M_{\tau+1:t}^{'\intercal} q')_{i!s''} \le \sum_{s \in S} q_{i!s} = \sum_{s \in S} \sum_{ \substack{i'!s \in [K]\times S \\ a \in A } } P_{t,i'!s,i!s'}^{'a} \\
    = \sum_{ s \in S, a \in A, s' \in S  } P_{t,i!s,i!s'}^{'a} = \sum_{ s,a,s' } P_{t,i,s,s'}^{a} = |S||A|.
\end{multline*}
Replacing this back into \eqref{eq:lm:stateError:boundt6} and noting that $\rmu'_{t+1,i|s} - \mmu'_{t+1,i|s} = \rmu_{t+1,i,s}= \mmu_{t+1,i,s}$, we have
\begin{equation}
    \Prob[ \rmu_{t+1} - \mmu_{t+1} \ge t|S|(|A| + \epsilon) ] \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)},
\end{equation}
for every $1 \le t \le T-1$ and $\epsilon > 0$. Following similar steps, we have
\begin{equation}
    \Prob[ \rmu_{t+1} - \mmu_{t+1} \le -t|S|(|A| + \epsilon) ] \le t \exp{ \left(- \frac{\epsilon^2}{2N} \right)},
\end{equation}
\end{proof}

==> old/analysis-10-16-22.tex <==


Remember that, in the previous section, we introduced an alternate way to represent the mean-field action called the normalized mean-field action $\mbeta$. This allowed us to plug in the mean-field action to the real-life system. In this section, to do the mathematical analysis, in addition to plugging in the mean-field action to the real-life system, we shall also plug in the real-life action to the mean-field system. To do so, we similarly compute a normalized real-life action $\rbeta$, defined below:

Let $\rbeta = (\rbeta_{t,i,s}^a)$ where $\rbeta_{t,i,s}^a = \ralpha_{t,i,s}^a / \rmu_{t,i,s}$ if $\rmu_{t,i,s} > 0$ and $\rbeta_{t,i,s} \in \Delta(A)$ (arbitrary) otherwise. Notice that $\rbeta_t$, like $\ralpha_t$, is also deterministic and Markov given $\rmu_t$. (But, as $\rmu_t$ is random, $\rbeta_t$ may also be random. $\rbeta_t$ becomes deterministic conditioned on $\rmu_t$.) 
% For $\xdot \in \{ \rdot, \mdot \}$, \AG{Maybe change this notation.} observe that there is a one-to-one mapping between $\xbeta$ and $\xalpha$ given $\xmu$, except when $\xmu_{t,i,s} = 0$. When $\xmu_{t,i,s} = 0$, any $\xbeta_{t,i,s} \in \Delta(A)$ will give $\xalpha_{t,i,s}^a = \xbeta_{t,i,s}^a \xmu_{t,i,s} = 0$ for every $a$. Also notice that $\xbeta$ satisfies $\xbeta_{t,i,s} \in \Delta(A)$ for every $t$, $i$, and $s$.
Observe that there is a one-to-one mapping between $\rbeta_{t,i,s}$ and $\ralpha_{t,i,s}$ given $\rmu_{t,i,s}$, except when $\rmu_{t,i,s} = 0$. When $\rmu_{t,i,s} = 0$, any $\rbeta_{t,i,s} \in \Delta(A)$ will give $\ralpha_{t,i,s}^a = \rbeta_{t,i,s}^a \rmu_{t,i,s} = 0$ for every $a$. Also notice that $\rbeta$ satisfies $\rbeta_{t,i,s} \in \Delta(A)$ for every $t$, $i$, and $s$.

% As $\ralpha_t$ and $\rbeta_t$ are deterministic Markov functions of the state $\rmu_t$, we should ideally write them as $\ralpha_t(\rmu_t)$ and $\rbeta_t(\rmu_t)$. % Essentially, $\ralpha_t(\rmu_t)$ and $\rbeta_t(\rmu_t)$ shall denote the deterministic Markov policies.

% Random stuff
% Say a finite horizon algorithm has error $\approx \frac{T^{3/2}}{\sqrt{N}}$ for some $a > 0$. For an infinite horizon problem with discount factor $\gamma < 1$, if we truncate at time $T$ then error $\approx \frac{T^{3/2}}{\sqrt{N}} + \gamma^T$. If we set $\gamma^T = \frac{1}{\sqrt{N}} \implies T = \frac{\log (N)}{2\log(1/\gamma)}$, then we get an overall error $\frac{poly(\log N)}{\sqrt{N}}$. On the other hand, if finite horizon error was $\frac{b^T}{\sqrt{N}}$ where $b > 1$, then infinite horizon error $\frac{b^T}{\sqrt{N}} + \gamma^T$, and the same trick does not work. If $b$ is quite small compared to $1/\gamma$ then we may get a bound of $1/N^c$ for some $c > 0$ but worse than $1/\sqrt{N}$. (If $b$ is sufficiently large, then no reasonable bound in $N$ is possible.) \cite{zhang2022near} does extend one of the finite horizon algorithms called fluid-balance to infinite horizon and have $1/\sqrt{N}$ bound. We get the same result essentially for free.

Let us pick an arbitrary start state $\mu_1 = (\mu_{1,i,s})$. Let $\beta = (\beta_{t,i,s}^a)$ be a sequence of normalized actions selected from an arbitrary Markov policy such that $\beta_{t,i,s} \in \Delta(A)$ for each $t$, $i$, and $s$. Notice that $\beta_t$ is allowed to be a function of $\rmu_t$. Given $\beta$ and $\mu_1$, we can define the real-life and mean-field process iteratively as:\\
For $t = 1, 2, \ldots, T-1$:
\begin{enumerate}
    \item The realization of $\beta_t = \pi(\rmu_t)$.
    \item The action at time $t$: 
    \begin{itemize}
        \item Mean-Field: $\malpha_t = (\malpha_{t,i,s}^a)$ where $\malpha_{t,i,s}^a = \beta_{t,i,s}^a  \mmu_{t,i,s}$.
        \item Real-Life: $\ralpha_t = (\ralpha_{t,i,s}^a)$ where $\ralpha_{t,i,s} = \round(\beta_{t,i,s}  \rmu_{t,i,s})$.
    \end{itemize}
    \item The state at time $t+1$: 
    \begin{itemize}
        \item Mean-Field: $\mmu_{t+1,i}^\intercal = \sum_{a \in A} \malpha_{t,i}^{a \intercal} P_i^a$.
        \item Real-Life: $\rmu_{t+1,i,s} = \sum_{s, a} \sum_{\ell \in [\ralpha_{t,i,s}^a]} \bI{\{x_{s,\ell}^a = s'\}}$  where $x_{s,\ell}^a \sim P_{t,i,s}^a$.
    \end{itemize}
\end{enumerate}
% If we want to be very specific, we may write $\malpha_t(\beta_t, \mmu_t)$ and $\mmu_{t+1}(\beta_t, \mmu_t)$ for the mean-field action and state, $\ralpha_t(\beta_t, \rmu_t)$ and $\rmu_{t+1}(\beta_t, \rmu_t)$ for the real-life action and state, and $\beta_t(\rmu_t)$ for the normalized action to highlight the functional dependency of the random variables. We shall suppress this notation to keep the exposition cleaner.

Given a start state $\mu_1$ and an arbitrary policy $\pi$, let $\rr(\mu_1, \pi)$ denote the expected real-life reward over the time horizon. Let $\mr(\mu_1, \pi)$ denote the reward estimated by the mean-field algorithm in \eqref{eq:mflp:1}.

Let us now state the main theorem of the paper.
\begin{theorem}\label{thm:}
Let $\mpi$ denote the mean-field policy and let $\rpi$ denote an optimal real-life policy. For any arbitrary start state $\mu_1$, TODO
\end{theorem}
\begin{proof}
There will be two main components of the proof, we show that (i) $\rr(\mu_1, \mpi) \approx \mr(\mu_1, \mpi)$ with high probability, (ii) $\mr(\mu_1, \mpi) \ge \rr(\mu_1, \rpi)$ almost surely. 

Let us pick an arbitrary deterministic Markov policy $\pi$ and corresponding sequence of normalized actions $\beta$. 

Notice that $\beta_{t,i}$ is an $|S| \times |A|$ right stochastic matrix for every $t$ and $i$. Similarly, $P_{t,i,s}$ is also a right stochastic matrix for every $t,i,s$. Let us define the $|S|\times|S|$ matrix $M_{t,i}$ as $M_{t,i,s,s'} = \sum_{a \in A} \beta_{t,i,s}^a P_{t,i,s,s'}^a$. $M_{t,i}$ is also a right stochastic matrix for every $t$ and $i$ because $\sum_{s'} M_{t,i,s,s'} = \sum_{s'} \sum_{a \in A} \beta_{t,i,s}^a P_{t,i,s,s'}^a = \sum_{a \in A} \beta_{t,i,s}^a \sum_{s'} P_{t,i,s,s'}^a = \sum_{a \in A} \beta_{t,i,s}^a = 1$.

At the initial time-point $t=1$, the real-life state and the mean-field state are both equal to $\mu_1$: $\rmu_1 = \mmu_1 = \mu_1$. At time $t$, there are two sources of divergence between the mean-field state $\mmu_{t}$ and the real-life state $\rmu_{t}$:
\begin{enumerate}
    \item Rounding. For each $t$, we do rounding to compute the real-life action $\ralpha_{t,i,s} = \round(\beta_{t,i,s} \rmu_{t,i,s})$, but not for the mean-field action $\malpha_{t,i,s} = \beta_{t,i,s} \mmu_{t,i,s}$. 
    % Notice that the rounding error may add bias.
    \item Randomness. The real-life state $\rmu_{t+1}$ is a random function of $\ralpha_t$ because of the stochasticity of the transitions.
\end{enumerate}
As mentioned, due to rounding, $\ralpha_{t,i,s}^a$ may not be equal to $\beta_{t,i,s}^a \rmu_{t,i,s}$. Let us define $\rbeta_{t,i,s}^a = \ralpha_{t,i,s}^a / \rmu_{t,i,s}$ if $\rmu_{t,i,s} > 0$ and $\rbeta_{t,i,s}^a = \beta_{t,i,s}^a$ otherwise. As we had defined the right stochastic matrix $M_{t,i}$ based on $\beta_{t,i}$ and $P_{t,i}$, we similarly define the $|S|\times|S|$ right stochastic matrix $\rM_{t,i} = (\sum_a \beta_{t,i,s}^a P_{t,i,s,s'}^a)_{s,s' \in S}$ based on $\rbeta_{t,i}$ and $P_{t,i}$.

Let us denote the matrix $\prod_{\ell = \tau}^{t} M_{\ell,i}$ as $M_{\tau:t,i}$ and the matrix $\prod_{\ell = \tau}^{t} \rM_{\ell,i}$ as $\rM_{\tau:t,i}$. If $\tau > t$, then let $M_{\tau:t,i}$ and $\rM_{\tau:t,i}$ be identity matrices. Using these matrices, the mean-field state can be rewritten as
\[
    \mmu_{t,i} = M_{1:t-1,i}^\intercal \mu_{1,i}.
\]

For $\pi$, the mean-field reward is
\begin{multline*}
    \mr(\mu_1,\pi) = \sum_{t \in T} \sum_{i \in [K]} \sum_{a \in A} R_{t,i}^{a \intercal} \malpha_{t,i}^a = \sum_{t,i,a} R_{t,i}^{a \intercal} (\beta_{t,i}^a \cdot \mmu_{t,i}) \\
    = \sum_{t,i} \left( \sum_a R_{t,i}^{a} \cdot \beta_{t,i}^a \right)^\intercal M_{1:t-1,i}^\intercal \mu_{1,i}.
\end{multline*}

Similarly, the real-life reward is
\[
    \rr(\mu_1, \pi) = \sum_{t,i,a} R_{t,i}^{a \intercal} \ralpha_{t,i}^a.
\]
As $\ralpha_{t,i,s} = \round(\beta_{t,i,s} \rmu_{t,i,s})$
\begin{multline*}
    \ralpha_{t,i,s}^a \in \{ \lfloor \rmu_{t,i,s} \beta_{t,i,s}^a \rfloor, \lceil \rmu_{t,i,s} \beta_{t,i,s}^a \rceil \} \\
    \implies -1 \le \ralpha_{t,i,s}^a - \rmu_{t,i,s} \beta_{t,i,s}^a \le 1.
\end{multline*}
Putting this back into the real-life reward
\begin{equation}
    \sum_{t,i,s,a} R_{t,i,s}^a \le \rr(\mu_1, \pi) - \sum_{t,i} \left( \sum_a R_{t,i}^{a} \cdot \beta_{t,i}^a \right)^\intercal \rmu_{t,i} \le \sum_{t,i,s,a} R_{t,i,s}^a.
\end{equation}
We can further bound $\sum_{t,i,s,a} R_{t,i,s}^a$ by $TK|S||A| R_{max}$, where $R_{max} = \max_{t,i,s,a} R_{t,i,s}^a$.

Let us now try to study the evolution of the real-life state $\mu_t$. Let $(\cF_{t})_{t \in [T]}$ denote the natural filtration with respect to $\rmu_t$, i.e., $\cF_{t}$ models the information available at time $t$. Notice that $\rmu_t$ is $\cF_t$-measurable by definition. 

\textbf{Let us focus on a particular time-step $t \rightarrow (t+1)$.} 
At time $t$, we know the realization of $\rmu_t$. Given $\rmu_t$, we know that $\beta_t$ is deterministic because $\pi$ is a deterministic Markov policy, and we also know that the action $\ralpha_{t,i,s} = \round(\beta_{t,i,s} \rmu_{t,i,s})$ is also deterministic because the rounding function and all the inputs to it are deterministic. 
Remember that $\ralpha_{t,i,s}^a$ is a non-negative integer and denotes the number of arms in cluster $i$ state $s$ at time $t$ for which we play action $a$. Also note that $\sum_{i,s,a} \ralpha_{t,i,s}^a = \sum_{i,s} \rmu_{t,i,s} = \sum_i N_i = N$ for every $t$.

Given $\rmu_t$, $\rmu_{t+1}$ is a random variable given by \\
$\rmu_{t+1,i,s'} = \sum_{s, a} \sum_{\ell \in [\ralpha_{t,i,s}^a]} \bI{\{z_{\ell,i,s}^a = s'\}}$ where $z_{\ell,i,s}^a \sim P_{t,i,s}^a$. To simplify notation for the upcoming analysis, let us enumerate the $N$ arms by $j = 1, 2, \ldots, N$ and denote arm $j$'s cluster, state, and action at time $t$ by $i_{j}$, $s_{t,j}$, and $a_{t,j}$ (cluster does not change with time). Let $\cN_i = \{ j \mid i_{j} = i\}$. Notice that, by definition, exactly $\ralpha_{t,i,s}^a$ arms will have cluster, state, and action equal to $i$, $s$ and $a$, respectively, i.e., $\sum_j \bI{\{i_j = i\}} \bI{\{s_{t,j} = s\}} \bI{\{a_{t,j} = a\}} = \ralpha_{t,i,s}^a$. 

Let $Z_{t+1,j}$ be the one-hot random variable that denotes the state of arm $j$ at time $t+1$; so, $(\arg\max_{s} Z_{t+1,j,s}) \sim P_{t,i_j,s_{t,j}}^{a_{t,j}}$. Notice that $Z_{t+1,j}$ for arm $j$ is picked independently of the other arms given $\rmu_t$. We can rewrite $\rmu_{t+1}$ as $\rmu_{t+1,i} = \sum_{j \in \cN_i} Z_{t+1,j}$. Further, $\Exp[\rmu_{t+1,i} \mid \cF_t]$ is 
\begin{multline*}
    \Exp[\rmu_{t+1,i} \mid \cF_t] = \Exp \left[ \left. \sum_{j \in \cN_i} Z_{t+1,j} \right| \cF_t \right] \\
    = \sum_{j \in \cN_i} \Exp [  Z_{t+1,j} \mid \cF_t ] = \sum_{j \in \cN_i} P_{t,i,s_j}^{a_j} \\ 
    = \sum_{s, a} \ralpha_{t,i,s}^a P_{t,i,s}^a = \sum_{s} \rmu_{t,i,s} \sum_a \rbeta_{t,i,s}^a P_{t,i,s}^a = \rM_{t,i}^\intercal \rmu_{t,i} .
\end{multline*}
On the other hand, given $\rmu_{t}$, if we were to estimate the expected value of the state at time $t+1$ without rounding, as done by the mean-field algorithm, then estimate of $\rmu_{t+1,i}$ would have been $\sum_{s,a} \rmu_{t,i,s} \beta_{t,i,s}^a P_{t,i,s}^a = M_{t,i}^\intercal \rmu_{t,i} $. So, the newly introduced rounding error in this transition between the real-life state and the mean-field estimated state, for cluster $i$, is
\[
    \rM_{t,i}^\intercal \rmu_{t,i} - M_{t,i}^\intercal \rmu_{t,i}.
\]

Let us now try to upper-bound the difference between real-life reward and the mean-field reward
\begin{align}
    &\rr(\mu_1, \pi) - \mr(\mu_1, \pi) = \sum_{t \in T} \sum_{i \in [K]} \sum_{a \in A} R_{t,i}^{a \intercal} (\ralpha_{t,i}^a - \malpha_{t,i}^a) \nonumber \\
    &\le \sum_{t,i} \left( \sum_a R_{t,i}^{a} \cdot \beta_{t,i}^a \right)^\intercal (\rmu_{t,i} - \mmu_{t,i}) + TK|S||A| R_{max}. \label{eq:thm:main:1}
\end{align}
Notice that $\beta_{t,i,s}$ is in $\Delta(A)$, therefore, for every $t,i,s$, $\sum_{a} R_{t,i,s}^a \beta_{t,i,s}^a \le \max_{a} R_{t,i,s}^a \le R_{max}$. Let us focus on the term $\sum_{t,i} \left( \sum_a R_{t,i}^{a} \cdot \beta_{t,i}^a \right)^\intercal (\rmu_{t,i} - \mmu_{t,i})$, we get
\begin{align*}
    &\sum_{t,i} \left( \sum_a R_{t,i}^{a} \cdot \beta_{t,i}^a \right)^\intercal (\rmu_{t,i} - \mmu_{t,i}) \le R_{max} \sum_{t,i} \b1^\intercal (\rmu_{t,i} - \mmu_{t,i}) \\
    &= R_{max}\b1^\intercal  \sum_{t,i} (\rmu_{t,i} - M_{1:t-1,i}^\intercal \mu_{1,i}) \\
    &= R_{max} \b1^\intercal \sum_{t,i} \sum_{\tau = 1}^{t-1}(M_{\tau+1:t-1,i}^\intercal \rmu_{\tau+1,i} - M_{\tau:t-1,i}^\intercal \rmu_{\tau,i}), \qquad \text{ telescope \MJ{?}} \\
    &= R_{max} \b1^\intercal \sum_{t,i} \sum_{\tau = 1}^{t-1} M_{\tau+1:t-1,i}^\intercal (\rmu_{\tau+1,i} - M_{\tau,i}^\intercal \rmu_{\tau,i}) \\
    &= R_{max} \b1^\intercal \sum_{t,i} \sum_{\tau = 1}^{t-1} M_{\tau+1:t-1,i}^\intercal ( (\rmu_{\tau+1,i} - \rM_{\tau,i}^\intercal \rmu_{\tau,i}) + (\rM_{\tau,i}^\intercal \rmu_{\tau,i} - M_{\tau,i}^\intercal \rmu_{\tau,i})),
\end{align*}
where the first term $R_{max} \b1^\intercal \sum_{t,i} \sum_{\tau = 1}^{t-1} M_{\tau+1:t-1,i}^\intercal (\rmu_{\tau+1,i} - \rM_{\tau,i}^\intercal \rmu_{\tau,i})$ captures the difference between the rewards due to randomness, and the second term $R_{max} \b1^\intercal \sum_{t,i} \sum_{\tau = 1}^{t-1} M_{\tau+1:t-1,i}^\intercal (\rM_{\tau,i}^\intercal \rmu_{\tau,i} - M_{\tau,i}^\intercal \rmu_{\tau,i})$ captures the difference in rewards due to rounding. First, let us focus on the rounding error. We provide an \textit{almost surely} bound for this error. As per our construction of the rounding function, we know that
\begin{multline}\label{eq:thm:main:2}
    \ralpha_{\tau,i,s}^a \in \{ \lfloor \rmu_{\tau,i,s} \beta_{\tau,i,s}^a \rfloor, \lceil \rmu_{\tau,i,s} \beta_{\tau,i,s}^a \rceil \} \\
    \implies - 1 \le \ralpha_{\tau,i,s}^a - \rmu_{\tau,i,s} \beta_{\tau,i,s}^a \le  + 1 \\
    \implies - \sum_{s, a} P_{\tau,i,s}^a \le \sum_{s, a} (\ralpha_{\tau,i,s}^a - \rmu_{\tau,i,s} \beta_{\tau,i,s}^a) P_{\tau,i,s}^a \le  \sum_{s, a}  P_{\tau,i,s}^a \\
    \implies -q_{\tau,i} \le \rM_{\tau,i}^\intercal \rmu_{\tau,i} - M_{\tau,i}^\intercal \rmu_{\tau,i} \le q_{\tau,i},
\end{multline}
where $q_{\tau,i}$ is the $|S|$-dimensional vector defined as $q_{\tau,i,s'} = \sum_{s, a}  P_{\tau,i,s,s'}^a$. Plugging this back into our total rounding error, we have
\begin{align*}
    & R_{max} \b1^\intercal \sum_{t,i} \sum_{\tau = 1}^{t-1} M_{\tau+1:t-1,i}^\intercal (\rM_{\tau,i}^\intercal \rmu_{\tau,i} - M_{\tau,i}^\intercal \rmu_{\tau,i}) \\
    & \le R_{max} \b1^\intercal \sum_{t,i} \sum_{\tau = 1}^{t-1} M_{\tau+1:t-1,i}^\intercal q_{\tau,i}.
\end{align*}
As $M_{\tau+1:t-1,i}$ is right stochastic, $\b1^\intercal (M_{\tau+1:t-1,i}^\intercal q_{\tau,i}) = \b1^\intercal q_{\tau,i} = |S| |A|$. Plugging this back, and also adding it with the error of $TK|S||A|R_{max}$ in \eqref{eq:thm:main:1}, we get the total rounding error to be 
\[
    \le T^2 K|S||A|R_{max}.
\]
Repeating the same steps, we can also get a lower bound of $- T^2 K|S||A|R_{max}$ for the rounding error.

Let us now look at the other error term, which is due to the randomness in the transitions, given by
\begin{multline*}
    R_{max} \b1^\intercal \sum_{t,i} \sum_{\tau = 1}^{t-1} M_{\tau+1:t-1,i}^\intercal (\rmu_{\tau+1,i} - \rM_{\tau,i}^\intercal \rmu_{\tau,i}) \\
    = R_{max} \b1^\intercal \sum_{\tau,i} \left( \sum_{t = \tau+1}^{T} M_{\tau+1:t-1,i}^\intercal \right) (\rmu_{\tau+1,i} - \rM_{\tau,i}^\intercal \rmu_{\tau,i})
    .
\end{multline*}
As discussed earlier, $\rmu_{\tau+1,i} = \sum_{j \in \cN_i} Z_{t+1,j}$ and $\Exp[\rmu_{\tau+1,i} \mid \cF_t] = \rM_{t,i}^\intercal \rmu_t$. Given $\cF_t$, the action $\ralpha_t$ is deterministic, therefore for each $j \in [N]$, $Z_{t+1,j}$ is picked independently based on $P_{t,i_j,s_{t,j}}^{a_{t,j}}$. So, we may hope to bound the $\rmu_{\tau+1,i} - \rM_{\tau,i}^\intercal \rmu_{\tau,i}$ terms, and subsequently, their sum using Azuma-Hoeffding (Lemma~\ref{lm:azuma}). But, the $\sum_{\tau,i} \left( \sum_{t = \tau+1}^{T} M_{\tau+1:t-1,i}^\intercal \right)$ term depends upon $\rmu_t$ for $t > \tau$, so $\sum_{\tau,i} \left( \sum_{t = \tau+1}^{T} M_{\tau+1:t-1,i_j}^\intercal \right) Z_{\tau+1,j}$ is no longer independent of \\
$\sum_{\tau,i} \left( \sum_{t = \tau+1}^{T} M_{\tau+1:t-1,i_{j'}}^\intercal \right) Z_{\tau+1,j'}$ for arbitrary $j$ and $j'$, and we cannot directly use Azuma--Hoeffding. In the remaining proof, we shall do three things
\MJ{we have to motivate why all this detail is necessary to cover all the corner cases.}
\begin{enumerate}
    \item Assuming $M_{t,i}$ is deterministic (and therefore independent of $\rmu_t$), we prove a tight bound using Azuma--Hoeffding.
    \item Relax the assumption and allow $M_{t,i}$ to be random and dependent on $\rmu_t$, we prove a weaker version of the bound.
    \item Tighten the weaker bound for the general case to the stronger bound derived for the deterministic case using properties of the mean-field algorithm.
\end{enumerate}
Let $Q_{\tau+1,i} = \frac{1}{T - \tau}\sum_{t = \tau+1}^{T} M_{\tau+1:t-1,i}^\intercal$. As $M_{\tau+1:t-1,i}$ is right stochastic for each $t$ and $\tau$, therefore $Q_{\tau+1,i}$ is left stochastic, i.e., each column of $Q_{\tau+1,i}$ is a probability distribution in $\Delta(S)$. As $Z_{\tau+1,j}$ is a one-hot vector, $Q_{\tau+1,i_j} Z_{\tau+1,j}$ is a (random) element in $\Delta(S)$. Further, $R_{max} \b1^\intercal Q_{\tau+1,i_j} Z_{\tau+1,j}$ is then a (random) element in $[0,R_{max}]$, i.e., it is bounded by $0$ and $R_{max}$. So, by Hoeffding's lemma (Lemma~\ref{lm:hoeffding}), $R_{max} \b1^\intercal (T-\tau) Q_{\tau+1,i_j} Z_{\tau+1,j} = R_{max} \b1^\intercal \left( \sum_{t = \tau+1}^{T} M_{\tau+1:t-1,i_j}^\intercal \right) Z_{\tau+1,j}$ is $((T-\tau)R_{max})^2/4$-subgaussian, and theerefore, is also $(T R_{max})^2/4$-subgaussian. 

\paragraph{$Q_{\tau,i}$ deterministic} Let us assume that $Q_{\tau,i}$ is deterministic, which happens, for example, when $\beta$ is the mean-field policy $\mbeta$, then $\beta_{\tau}$ is deterministic and does not depend upon $\rmu_{\tau}$, then $M_{\tau,i}$ (a function of $\beta_{\tau,i}$ and $P_{\tau,i}$) is also deterministic, then so is $Q_{\tau,i}$. In this case,
\begin{multline*}
    \Exp[ R_{max} \b1^\intercal (T-\tau) Q_{\tau+1,i_j} (Z_{\tau+1,j} - P_{t,i_j,s_{t,j}}^{a_{t,j}}) \mid \cF_{\tau}] \\
    = R_{max} \b1^\intercal (T-\tau) Q_{\tau+1,i_j} \Exp[ Z_{\tau+1,j} - P_{t,i_j,s_{t,j}}^{a_{t,j}} \mid \cF_{\tau}] = 0.
\end{multline*}
Also, the term $R_{max} \b1^\intercal (T-\tau) Q_{\tau+1,i_j} (Z_{\tau+1,j} - P_{t,i_j,s_{t,j}}^{a_{t,j}})$ is $\cF_{\tau+1}$ measurable. So, we can apply the Azuma-Hoeffding inequality and get
\begin{multline}\label{eq:thm:main:2.1}
   \Prob[R_{max} \b1^\intercal \sum_{\tau,i} \left( \sum_{t = \tau+1}^{T} M_{\tau+1:t-1,i}^\intercal \right) (\rmu_{\tau+1,i} - \rM_{\tau,i}^\intercal \rmu_{\tau,i}) \ge \epsilon] \\
   = \Prob[\sum_{\tau \in [T]} \sum_{j \in [N]} R_{max} \b1^\intercal (T-\tau) Q_{\tau+1,i_j} (Z_{\tau+1,j} - P_{t,i_j,s_{t,j}}^{a_{t,j}}) \ge \epsilon] \\
   \le \exp{\left( \frac{-2\epsilon^2}{N T^3 R_{max}^2} \right)}.
\end{multline}
In particular, notice that we can use this and the rounding error bound to bound the total error between $\rr(\mu_1,\mpi)$ and $\mr(\mu_1,\mpi)$ because the mean-field policy $\mpi$ leads to deterministic $Q_{\tau,i}$ matrices. In particular, we can write the following lower bound on  $\rr(\mu_1,\mpi)$ 
\begin{multline}\label{eq:thm:main:2.2}
    \Prob[\rr(\mu_1, \mpi) - \mr(\mu_1, \mpi) \le -\epsilon - T^2 K |S| |A| R_{max}] \\
    \le \exp{\left( \frac{-2\epsilon^2}{N T^3 R_{max}^2} \right)}.
\end{multline}

\paragraph{$Q_{\tau,i}$ can be a function of $\rmu_t$ for any $t$} We will prove a bound by taking a supremum over approximately all possible values of $Q_{\tau,i}$ for each $\tau$ and $i$. $Q_{\tau,i}$ is an element in $\Delta(S)^{|S|}$. Let us discretize this $|S|\times|S|$ space where each element of the matrix can take values in $E = \{0, \eta, 2\eta, \ldots, 1-\eta, 1\}$. For any $Q_{\tau,i}$, we can find an approximate $Q_{\tau,i}'$ such that $Q_{\tau,i,s,s'}' \in E$ and $-\eta \le Q_{\tau,i,s,s'} - Q_{\tau,i,s,s'}' \le \eta$ (we can use a rounding scheme similar to our $\round(\ldots)$ function). So,
\begin{multline*}
    -2R_{max}T|S|\eta \\
    \le R_{max} \b1^\intercal (T-\tau) (Q_{\tau+1,i_j} - Q_{\tau+1,i_j}') (Z_{\tau+1,j} - P_{t,i_j,s_{t,j}}^{a_{t,j}}) \\
    \le 2R_{max}T|S|\eta.
\end{multline*}
Putting these ideas together and using union bound we get
\begin{align*}
    &\Prob[\sum_{\tau \in [T]} \sum_{j \in [N]} R_{max} \b1^\intercal (T-\tau) Q_{\tau+1,i_j} (Z_{\tau+1,j} - P_{t,i_j,s_{t,j}}^{a_{t,j}}) \ge \epsilon] \\
    &\le \sup_{Q_{\tau+1,i} \in \Delta(S)^{|S|}} \Prob[\sum_{\tau,j} R_{max} \b1^\intercal (T-\tau) Q_{\tau+1,i_j} \\
    & \qquad (Z_{\tau+1,j} - P_{t,i_j,s_{t,j}}^{a_{t,j}}) \ge \epsilon] \\
    &\le \sup_{Q'_{\tau+1,i} \in E^{|S|\times|S|} \cap \Delta(S)^{|S|}} \Prob[\sum_{\tau,j} R_{max} \b1^\intercal (T-\tau) Q'_{\tau+1,i_j} \\
    & \qquad (Z_{\tau+1,j} - P_{t,i_j,s_{t,j}}^{a_{t,j}}) \ge \epsilon + 2R_{max}T^2|S| N\eta] \\
    & \qquad \qquad \le \left(1+\frac{1}{\eta}\right)^{KT|S|^2} \exp{\left( \frac{-2\epsilon^2}{N T^3 R_{max}^2} \right)}.
\end{align*}
For example, if we set $\epsilon = N^{2/3}/2$ and $\eta = 1/(4 R_{max} T^2 |S| N^{1/3})$, then we get
\begin{multline}\label{eq:thm:main:3}
    \Prob[\sum_{\tau,j} R_{max} \b1^\intercal (T-\tau) Q_{\tau+1,i_j} (Z_{\tau+1,j} - P_{t,i_j,s_{t,j}}^{a_{t,j}}) \ge N^{2/3}] \\
    = \Prob[R_{max} \b1^\intercal \sum_{\tau,i} \left( \sum_{t = \tau+1}^{T} M_{\tau+1:t-1,i}^\intercal \right) (\rmu_{\tau+1,i} - \rM_{\tau,i}^\intercal \rmu_{\tau,i}) \ge N^{2/3}] \\
    \le (8 R_{max} T |S| N^{1/3} )^{TK|S|^2} \exp{\left( \frac{-N^{1/3}}{2T^3 R_{max}^2} \right)}.
\end{multline}
There are two main observations in the result in \eqref{eq:thm:main:3}: (i)
as $N \rightarrow \infty$, the probability of not satisfying the error bound goes to $0$: $(8 R_{max} T |S| N^{1/3} )^{TK|S|^2} \exp{\left( \frac{-N^{1/3}}{2T^3 R_{max}^2} \right)} \rightarrow 0$; (ii) the error bound of $N^{2/3}$ is sub-linear in $N$.

We can similarly derive a symmetric lower bound.

\paragraph{Making copies trick \MJ{Need to motivate this as a way to reduce error}} 
Combining the randomness error in \eqref{eq:thm:main:3} with the rounding error of $T^2 K|S||A|R_{max}$, we get that 
\begin{multline}\label{eq:thm:main:4}
    \Prob[|\rr(\mu_1, \pi) - \mr(\mu_1, \pi)| \ge N^{2/3} + T^2 K|S||A|R_{max}] \\
    \le 2 (8 R_{max} T |S| N^{1/3} )^{TK|S|^2} \exp{\left( \frac{-N^{1/3}}{2T^3 R_{max}^2} \right)}.
\end{multline}
Based on the arbitrary RMAB instance we are currently working with, consider the following four scenarios:
\MJ{this could benefit from a table or a pictorial representation as well}
\begin{enumerate}
    \item Make $m$ copies of each arm, and also scale the budget and the start state by $m$. Everything else---clusters, transitions probabilities, rewards, costs, etc.--- remain the same. It is easy to see that the mean-field LP is equivalent as before, just the terms have been scaled by a constant. If we take an optimal solution of the original LP and multiple it by $m$, it will be optimal for the large LP, and on the reverse directions, if we take an optimal solution of the large LP and divide it by $m$, then we will get an optimal solution of the original LP. Let's say the optimal mean-field reward for this large LP be $r_{1,m}$, notice that $r_{1,m} = m \mr(\mu_1, \mpi)$.
    \item For the enlarged RMAB with $m$ copies of the original RMAB problem, as discussed in the previous point, find the optimal real-life policy. Let's denote this reward by $r_{2,m}$.
    \item For the enlarged RMAB with $m$ copies of the original RMAB problem, as discussed earlier, run the optimal policy for the original small RMAB in each of the $m$ copies. Let's call this reward $r_{3,m}$. Notice that by definition $r_{3,m} = m \rr(\mu_1, \rpi)$.
    \item For the mean-field LP corresponding to the large RMAB, let $r_{4,m}$ denote the mean-field reward if we were to plug in the optimal real-life policy for the large RMAB to the mean-field reward computation (i.e., of the form $\mr(\mu_1,\rpi)$ adapted to the larger RMAB). This reward will be at most that of using the mean-field policy, because the mean-field policy explicitly optimizes the LP. So, $r_{1,m} \ge r_{4,m}$
\end{enumerate}
Now, by definition $r_{2,m}$ is optimal for the large RMAB, so $r_{2,m} \ge r_{3,m} = m \mr(\mu_1, \rpi)$. Now, using the bound in \eqref{eq:thm:main:4} for the large RMAB, we can compare $r_{1,m}$ and $r_{2,m}$ as
\begin{multline*}
    \Prob[r_{2,m} - r_{4,m} \ge N^{2/3} m^{2/3} + T^2 K|S||A|R_{max}] \\
    \le 2 (8 R_{max} T |S| N^{1/3} m^{1/3} )^{TK|S|^2} \exp{\left( \frac{-N^{1/3} m^{1/3}}{2T^3 R_{max}^2} \right)}.
\end{multline*}
Now, as $r_{2,m} \ge  r_{3,m}$ and $r_{1,m} \ge  r_{4,m}$, therefore $r_{3,m} - r_{1,m} \le r_{2,m} - r_{4,m}$. Plugging this in, we get
\begin{multline*}
    \implies \Prob[ \rr(\mu_1, \rpi) - \mr(\mu_1, \mpi) \ge N^{2/3} m^{-1/3} + T^2 K|S||A|R_{max} m^{-1}] \\
    \le 2 (8 R_{max} T |S| N^{1/3} m^{1/3} )^{TK|S|^2} \exp{\left( \frac{-N^{1/3} m^{1/3}}{2T^3 R_{max}^2} \right)}.
\end{multline*}
Now, let $m \rightarrow \infty$. The probability of making an error outside the bound goes to zero, i.e., $\lim_{m \rightarrow \infty} 2 (8 R_{max} T |S| N^{1/3} m^{1/3} )^{TK|S|^2} \exp{\left( \frac{-N^{1/3} m^{1/3}}{2T^3 R_{max}^2} \right)} = 0$. Further, the error bound also goes to $0$, i.e., $\lim_{m \rightarrow \infty} N^{2/3} m^{-1/3} + T^2 K|S||A|R_{max} m^{-1} = 0$. So, $\rr(\mu_1, \rpi) \le \mr(\mu_1, \mpi)$ almost surely. Combining this with \eqref{eq:thm:main:2.2}, we get
\begin{multline*}
    \Prob[\rr(\mu_1, \mpi) - \rr(\mu_1, \rpi) \le -\epsilon - T^2 K |S| |A| R_{max}] \\
    \le \exp{\left( \frac{-2\epsilon^2}{N T^3 R_{max}^2} \right)}.
\end{multline*}
If we set the probability of making large error to be $\delta$, then $\exp{\left( \frac{-2\epsilon^2}{N T^3 R_{max}^2} \right)} = \delta \implies \epsilon = \frac{R_{max} T^{3/2 \sqrt{N}}}{2} \log(\frac{1}{\delta})$. So, with probability $1-\delta$, 
\[
    \rr(\mu_1, \mpi) \ge \rr(\mu_1, \rpi) - \frac{R_{max} T^{3/2} \sqrt{N}}{2} \log{\left(\frac{1}{\delta} \right)} - R_{max} T^2 K |S| |A|.
\]

\AG{The entire analysis was assuming the discount factor $\gamma = 1$.} \MJ{We should mention this ahead, and talk about how the discount factor would change the analysis -- although showing in math may not be necessary.}
    
\end{proof}





% In the next lemma, we show that with high probability $\rmu_t$ is close to $\mmu_t$ and $\ralpha_t$ is close to $\malpha_t$ where $\rmu_t$, $\mmu_t$, $\ralpha_t$, and $\malpha_t$ are as described above based on $\mu_1$ and $\beta$, for any $\mu_1$ and $\beta$.

% \begin{lemma}\label{lm:stateBound}
% % For any Markov normalized action sequence $\beta$, let $\rmu_{t}$ and $\mmu_{t}$ denote the real-life and mean-field state at time $t$. 
% For every $t \in [T-1]$, for every cluster $i \in [K]$, for every $\epsilon_i > 0$,
% \begin{align*}
%     \Prob[ \rmu_{t+1,i} - \mmu_{t+1,i} \ge_{any} t|S|(|A| + \epsilon_i) ] \le t |S|\exp{ \left(- \frac{2\epsilon_i^2}{N_i} \right)}, \\
%     \Prob[ \rmu_{t+1,i} - \mmu_{t+1,i} \le_{any} -t|S|(|A| + \epsilon_i) ] \le t |S|\exp{ \left(- \frac{2\epsilon_i^2}{N_i} \right)}.
% \end{align*}
% \AG{Actually, the probability bound is true for all $\tau \le t$ with the same probability bound, i.e., we need not use union bound over t again.}
% \end{lemma}
% \begin{proof}






% In the next segment of the proof, we will try to measure how much \textit{new} error is introduced between the mean-field estimate and the real-life process in a given time step due to rounding and randomness. Later in the proof, we shall  quantify how this error gets accumulated over time. 




% % Adding the error in \eqref{eq:lm:stateError:roundBound2} across all clusters, we get
% % \begin{equation}
% %     -\sum_{i} q_i \le \sum_i \rM_{t,i}^\intercal \rmu_{t,i} - \sum_i M_{t,i}^\intercal \rmu_{t,i} \le \sum_i q_i.
% % \end{equation}

% Next, let us focus on the divergence between $\rmu_{t+1,i}$ and  $\Exp[\rmu_{t+1,i} \mid \cF_t] = \rM_{t,i}^\intercal \rmu_{t,i}$. We shall show that $\rmu_{t+1,i}$ is close to $\rM_{t,i}^\intercal \rmu_{t,i}$ with high probability.

% Given $\mu_t$, for each arm $j$, $Z_j$ is sampled independently. Also note that $0 \le Z_{j,s} \le 1$ for every $s$. Applying Hoeffding's inequality (Lemma~\ref{lm:hoeffding}) for beneficiaries in cluster $i$, for each $s \in S$ we have
% \begin{equation*}
%     \Prob \left[ \sum_{j \in \cN_i} Z_{j,s} - (\rM_{t,i}^\intercal \rmu_{t,i})_s \ge \epsilon_i \right] \le \exp{ \left(- \frac{2\epsilon_i^2}{N_i} \right)}.
% \end{equation*}
% Applying union bound for every $s \in S$, we get
% \begin{equation}\label{eq:lm:stateError:2}
%     \Prob \left[ \sum_{j \in \cN_i} Z_j - \rM_{t,i}^\intercal \rmu_{t,i} \ge_{any} \epsilon_i  \right] \le |S|\exp{ \left(- \frac{2\epsilon_i^2}{N_i} \right)}.
% \end{equation}
% We know that $\sum_{j \in \cN_i} Z_j = \rmu_{t+1,i}$. Combining \eqref{eq:lm:stateError:1} with \eqref{eq:lm:stateError:2}, we have
% \begin{equation}\label{eq:lm:stateError:3}
%     \Prob \left[\rmu_{t+1,i} -  M_{t,i}^\intercal \rmu_{t,i} \ge_{any} \epsilon_i + q_{t,i} \right] \le |S|\exp{ \left(- \frac{2\epsilon_i^2}{N_i} \right)}.
% \end{equation}
% The bound in \eqref{eq:lm:stateError:3} is true for all $t \ge 1$. Let us pick a time $\tau \le t$. If $\rmu_{\tau+1,i} - M_{\tau,i}^\intercal \rmu_{\tau,i} <_{all} q_{\tau,i} + \epsilon_i$, then multiplying both sides by $\left(\prod_{\ell = \tau+1}^{t} M_{\ell,i} \right)^\intercal$ we have
% \begin{equation}\label{eq:lm:stateError:4}
%     \left(\prod_{\ell = \tau+1}^{t} M_{\ell,i} \right)^\intercal \rmu_{\tau+1,i} - \left(\prod_{\ell = \tau}^{t} M_{\ell,i} \right)^\intercal \rmu_{\tau,i} <_{all} \left(\prod_{\ell = \tau+1}^{t} M_{\ell,i} \right)^\intercal (q_{\tau,i} + \b1 \epsilon_i ),
% \end{equation}
% where $\b1$ is the vector of all ones. Let us denote the matrix $\prod_{\ell = \tau}^{t} M_{\ell,i}$ as $M_{\tau:t,i}$. As $M_{\ell,i}$ is right stochastic for every $\ell$, $M_{\tau:t,i}$ is also right stochastic. Combining equations \eqref{eq:lm:stateError:3} and \eqref{eq:lm:stateError:4} for $\tau = 1, \ldots, t$ and applying union-bound we get
% \begin{multline*}
%     \Prob \left[ \sum_{\tau = 1}^{t} (M_{\tau+1:t,i}^\intercal \rmu_{\tau+1,i} - M_{\tau:t,i}^\intercal \rmu_{\tau,i}) \right. \\
%     \left. \ge_{any} \sum_{\tau = 1}^{t}  M_{\tau+1:t,i}^\intercal (q_{\tau,i} + \b1 \epsilon_i ) \right] \le t |S| \exp{ \left(- \frac{2\epsilon_i^2}{N_i} \right)}.
% \end{multline*}
% Notice that sum $\sum_{\tau = 1}^{t} (M_{\tau+1:t,i}^\intercal \rmu_{\tau+1,i} - M_{\tau:t,i}^\intercal \rmu_{\tau,i})$ is telescoping and is equal to $\rmu_{t+1,i} - M_{1:t,i}^\intercal \rmu_{1,i}$. Notice that $\rmu_1 = \mu_1 = \mmu_1$, and by definition, the mean-field state at time $t+1$ is $\mmu_{t+1,i} = M_{1:t,i}^\intercal \mmu_{1,i}$. So, we get 
% \begin{equation}\label{eq:lm:stateError:5}
%     \Prob \left[ \rmu_{t+1,i} - \mmu_{t+1,i} \ge_{any} \sum_{\tau = 1}^{t}  M_{\tau+1:t,i}^\intercal (q_{\tau,i} + \b1 \epsilon_i ) \right] \le t |S| \exp{ \left(- \frac{2\epsilon_i^2}{N_i} \right)}.
% \end{equation}
% Let us now try to bound the error term: $\sum_{\tau = 1}^{t}  M_{\tau+1:t,i}^\intercal (q_{\tau,i} + \b1 \epsilon_i )$. As $M_{\tau+1:t,i}$ is right stochastic, every element of the matrix is $\le 1$, and therefore, $M_{\tau+1:t,i}^\intercal q_{\tau,i} \le \sum_{s'} q_{\tau,i,s'} = \sum_{s,a,s'} P_{\tau,i,s,s'}^a = |S||A|$ and $M_{\tau+1:t,i}^\intercal \b1 \epsilon_i \le \epsilon_i |S|$. Putting it back to \eqref{eq:lm:stateError:5} we get
% \begin{equation}\label{eq:lm:stateError:6}
%     \Prob[ \rmu_{t+1,i} - \mmu_{t+1,i} \ge_{any} t|S|(|A| + \epsilon_i) ] \le t |S|\exp{ \left(- \frac{2\epsilon_i^2}{N_i} \right)},
% \end{equation}
% for every $t \in [T-1]$, $i \in [K]$ and $\epsilon_i > 0$. Following analogous steps, we get
% \begin{equation}\label{eq:lm:stateError:7}
%     \Prob[ \rmu_{t+1,i} - \mmu_{t+1,i} \le_{any} -t|S|(|A| + \epsilon_i) ] \le t |S|\exp{ \left(- \frac{2\epsilon_i^2}{N_i} \right)},
% \end{equation}
% for every $t \in [T-1]$, $i \in [K]$ and $\epsilon_i > 0$. 
% \end{proof}

% The previous lemma bounds the difference between the mean-field state and the real-life state at any time $t$ with high probability. Next, we use this lemma to give a similar bound for rewards. We shall give two versions of this bound.

% Most of the application domains for RMABs have homogeneous rewards functions across all arms, i.e., $R_{t,i,s}^a = R_{t,i',s}^a$ for every $i,i' \in [K]$ and for every  $t$, $s$, and $a$. If a given RMAB satisfies this condition, or an approximate version of this condition of the form $R_{t,i,s}^a \le \eta R_{t,i',s}^a$ for every $i,i' \in [K]$, for some constant $\eta$, then we can bound the (leading term of the) error between mean-field and optimal expected reward by a factor proportional to $\sqrt{K}$. Even if the rewards are not exactly homogeneous, the approximate version of homogeneity may be easy to satisfy by introducing a small number of additional states (compared to $K|S|$). 

% We shall also provide an error bound with no assumptions about the reward function, and the bound is proportional to $K$.

% \begin{lemma}\label{lm:rewardBound1}
% Let the reward functions satisfy the following homogeneity condition across arms:
% \[
%     R_{t,i,s}^a \le \eta R_{t,i',s}^a, \qquad \text{for every $t \in [T], i,i' \in [K], s \in S, a \in A$},
% \]
% for some constant $\eta$. Then,

% \end{lemma}
% \begin{proof}
% Lemma~\ref{lm:stateBound} provided a high-probability error bound between $\rmu_{t+1,i}$ and $\mmu_{t+1,i}$. Let us use it provide a similar bound between $\sum_i \rmu_{t+1,i}$ and $\sum_i \mmu_{t+1,i}$. 
% \end{proof}


==> old/hard-examples-10-16-22.tex <==
\begin{proof}
\textbf{Whittle Index for the Reliable arm: }
By the definition of q-value, we have:
\begin{equation}\label{eq:trickyForWhittle:1}
    % Q^{rl}_{\lambda}(str, 0) = \gamma \max_{a} Q^{rl}_{\lambda}(drp, a),
    Q^{rl}_{\lambda}(s_0, 0) = \gamma \max_{a} Q^{rl}_{\lambda}(s_d, a),
\end{equation}
\begin{equation}\label{eq:trickyForWhittle:2}
    Q^{rl}_{\lambda}(s_0, 1) = - \lambda + \gamma \max_{a} Q^{rl}_{\lambda}(s_e, a).
\end{equation}
Notice that for the dropout state,
\begin{equation}\label{eq:trickyForWhittle:3}
    Q^{rl}_{\lambda}(s_d, 0) = \gamma \max_{a} Q^{rl}_{\lambda}(s_d, a), 
\end{equation}
\begin{equation}\label{eq:trickyForWhittle:4}
    Q^{rl}_{\lambda}(s_d, 1) = - \lambda + \gamma \max_{a} Q^{rl}_{\lambda}(s_d, a).
\end{equation}
% As $\lambda \ge 0$, we have $Q^{rl}_{\lambda}(drp, 0) \ge Q^{rl}_{\lambda}(drp, 1)$. Plugging this into \eqref{eq:trickyForWhittle:3}, we get
As $\lambda \ge 0$, we have $Q^{rl}_{\lambda}(s_d, 0) \ge Q^{rl}_{\lambda}(s_d, 1)$. Plugging this into \eqref{eq:trickyForWhittle:3}, we get
\begin{equation}\label{eq:trickyForWhittle:5}
    \max_{a} Q^{rl}_{\lambda}(s_d, a) = Q^{rl}_{\lambda}(s_d, 0) = 0.
\end{equation}

Let us denote $\max_{a} Q^{rl}_{\lambda}(s_e, a)$ by the variable $x$. We can rewrite the equations \eqref{eq:trickyForWhittle:1} and \eqref{eq:trickyForWhittle:2} for the q-values of the start state, using $x$ and equation \eqref{eq:trickyForWhittle:5}, as:
\begin{equation}\label{eq:trickyForWhittle:6}
    Q^{rl}_{\lambda}(s_0, 0) = 0; \quad Q^{rl}_{\lambda}(s_0, 1) = - \lambda + \gamma x.
\end{equation}

Now, for the engaged state, we similarly get
\begin{equation}\label{eq:trickyForWhittle:7}
    Q^{rl}_{\lambda}(s_e, 0) = (1-\epsilon) + \gamma \max_{a} Q^{rl}_{\lambda}(s_d, a) = (1-\epsilon),
\end{equation}
\begin{equation}\label{eq:trickyForWhittle:8}
    Q^{rl}_{\lambda}(s_e, 1) = (1-\epsilon) - \lambda + \gamma \max_{a} Q^{rl}_{\lambda}(s_e, a) = (1-\epsilon) - \lambda + \gamma x.
\end{equation}

If $\lambda$ is the Whittle index for the start state for the beneficiary, then
\begin{equation}\label{eq:trickyForWhittle:9}
    Q^{rl}_{\lambda}(s_0, 0) = Q^{rl}_{\lambda}(s_0, 1) \implies \lambda = \gamma x.
\end{equation}
Replacing this in \eqref{eq:trickyForWhittle:8}, we have
\begin{multline}\label{eq:trickyForWhittle:10}
    Q^{rl}_{\lambda}(s_e, 1) = (1-\epsilon) - \lambda + \gamma x = (1-\epsilon) = Q^{rl}_{\lambda}(s_e, 0) \\
    \implies x = \max_{a} Q^{rl}_{\lambda}(s_e, a) = (1-\epsilon) \implies \lambda = \gamma (1-\epsilon).
\end{multline}
So, the Whittle index for the start state for the reliable arm is $\gamma (1-\epsilon)$.

\textbf{Whittle Index for the Greedy arm: }
For the dropout state, as before, we have 
\[ Q^{gr}_{\lambda}(s_d, 0) = \gamma \max_{a} Q^{gr}_{\lambda}(s_d, a), \]
\[ Q^{gr}_{\lambda}(s_d, 1) = - \lambda + \gamma \max_{a} Q^{gr}_{\lambda}(s_d, a).\]
As $\lambda \ge 0$, we have $Q^{gr}_{\lambda}(s_d, 0) \ge Q^{gr}_{\lambda}(s_d, 1) \implies \max_{a} Q^{gr}_{\lambda}(s_d, a) = Q^{gr}_{\lambda}(s_d, 0) = 0$. Now, for the engaged state, 
\[ Q^{gr}_{\lambda}(s_e, 0) = 1 + \gamma \max_{a} Q^{gr}_{\lambda}(s_d, a) = 1, \]
\[ Q^{gr}_{\lambda}(s_e, 1) = 1 - \lambda + \gamma \max_{a} Q^{gr}_{\lambda}(s_d, a) = 1 - \lambda.\]
As $\lambda \ge 0$, we have $\max_{a} Q^{gr}_{\lambda}(s_e, a) = 1$. 
Finally, for the start state,
\[ Q^{gr}_{\lambda}(s_0, 0) = \gamma \max_{a} Q^{gr}_{\lambda}(s_d, a) = 0, \]
\[ Q^{gr}_{\lambda}(s_0, 1) = - \lambda + \gamma \max_{a} Q^{gr}_{\lambda}(s_e, a) = - \lambda + \gamma.\]
If $\lambda$ is the Whittle index for the start state for the beneficiary, then
\[
    Q^{gr}_{\lambda}(s_0, 0) = Q^{gr}_{\lambda}(s_0, 1) \implies \lambda = \gamma.
\]
So, the Whittle index for the start state for the greedy arm is $\gamma$.
\end{proof}

\MJ{It feels hard to follow. Let's think how we can simplify the presentation more.} \DN{We should also consider relegating some of the calculations to the appendix and state something like "Solving these equations gives so and so as the whittle index"} \AG{The proof has been updated - it now also proves indexability and is a bit easier to read.}
